Data-Driven Materials Discovery and Synthesis using Machine Learning Methods

Experimentally [1-38] and computationally [39-50] validated machine learning (ML) articles are sorted based on the size of the training data: 1-100, 101-10000, and 10000+ in a comprehensive set summarizing legacy and recent advances in the field. The review emphasizes the interrelated fields of synthesis, characterization, and prediction. Size range 1-100 consists mostly of Bayesian optimization (BO) articles, whereas 101-10000 consists mostly of support vector machine (SVM) articles. The articles often use combinations of ML, feature selection (FS), adaptive design (AD), high-throughput (HiTp) techniques, and domain knowledge to enhance predictive performance and/or model interpretability. Grouping cross-validation (G-CV) techniques curb overly optimistic extrapolative predictive performance. Smaller datasets relying on AD are typically able to identify new materials with desired properties but do so in a constrained design space. In larger datasets, the low-hanging fruit of materials optimization is typically already discovered, and the models are generally less successful at extrapolating to new materials, especially when the model training data favors a particular type of material. The large increase of ML materials science articles that perform experimental or computational validation on the predicted results demonstrates the interpenetration of materials informatics with the materials science discipline and an accelerating materials discovery for real-world applications.

==> tables/tab-comp-exp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}
\centering
\caption{Number of experimental and computational articles within each dataset size range, including references.}
\label{tab:comp-exp}
\begin{tabular}{@{}clll@{}}
\cmidrule(l){2-4}
\multicolumn{1}{l}{} &
  \multicolumn{3}{c}{Dataset Size} \\ \cmidrule(l){2-4} 
 &
  \multicolumn{1}{c}{\numrange{1}{100}} &
  \multicolumn{1}{c}{\numrange{101}{10000}} &
  \multicolumn{1}{c}{\num{10000}+} \\ \midrule
Computationally   Validated &
  4   (\cite{balachandranDatadrivenDesignB202020,balachandranLearningDataDesign2017,balachandranPredictingDisplacementsOctahedral2017,talapatraAutonomousEfficientExperiment2018}) &
  1   (\cite{sekoMatrixTensorbasedRecommender2018}) &
  2   (\cite{meredigCombinatorialScreeningNew2014,parkDevelopingImprovedCrystal2020}) \\
Experimentally Validated &
  13   (\cite{beraIntegratedComputationalMaterials2014,chenMachineLearningAssisted2020,hommaOptimizationHeterogeneousTernary2020,houMachineLearningAssistedDevelopmentTheoretical2019,iwasakiIdentificationAdvancedSpindriven2019,liEfficientOptimizationPerformance2018,rickmanMaterialsInformaticsScreening2019,shampDecompositionProductsPhosphine2016,wahabMachinelearningassistedFabricationBayesian2020,wakabayashiMachinelearningassistedThinfilmGrowth2019,wengSimpleDescriptorDerived2020,wuMachinelearningassistedDiscoveryPolymers2019,xueAcceleratedSearchBaTiO3based2016}) &
  15   (\cite{balachandranExperimentalSearchHightemperature2018,buciorEnergybasedDescriptorsRapidly2019,caoHowOptimizeMaterials2018,gzylHalfHeuslerStructuresFullHeusler2020,gzylSolvingColoringProblem2019,kauweMachineLearningPrediction2018,oliynykDisentanglingStructuralConfusion2017,oliynykHighThroughputMachineLearningDrivenSynthesis2016,raccugliaMachinelearningassistedMaterialsDiscovery2016,renAcceleratedDiscoveryMetallic2018,tehraniMachineLearningDirected2018,wenMachineLearningAssisted2019,yanOptimizationThermalConductivity2020,zhuoEvaluatingThermalQuenching2020,zhuoIdentifyingEfficientThermally2018}) &
  2   (\cite{buciorEnergybasedDescriptorsRapidly2019,gaultoisPerspectiveWebbasedMachine2016,yuanAcceleratedDiscoveryLarge2018}) \\ \bottomrule
\end{tabular}
\end{table}

==> tables/tab-ml-type.tex <==
\begin{table}[]
\centering
\caption{Number of articles for \acrfull{bo}, \acrfull{svm}, \acrfull{sr}, \acrfull{rf}, \acrfull{dt}, ensemble, \acrfull{ann}, \acrfull{lasso}, \acrfull{lr}, \acrfull{pr}, and \acrfull{pls} within each dataset size range, including references.}
\label{tab:ml-type}
\begin{tabular}{clll}
\cline{2-4}
\multicolumn{1}{l}{} &
  \multicolumn{3}{c}{Dataset Size} \\ \cline{2-4} 
\acrshort{ml} Type &
  \multicolumn{1}{c}{1-100} &
  \multicolumn{1}{c}{101-10000} &
  \multicolumn{1}{c}{10000+} \\ \hline
\acrshort{bo} &
  9   (\cite{hommaOptimizationHeterogeneousTernary2020,houMachineLearningAssistedDevelopmentTheoretical2019,iwasakiIdentificationAdvancedSpindriven2019,liEfficientOptimizationPerformance2018,talapatraAutonomousEfficientExperiment2018,wahabMachinelearningassistedFabricationBayesian2020,wakabayashiMachinelearningassistedThinfilmGrowth2019,wuMachinelearningassistedDiscoveryPolymers2019,xueAcceleratedSearchBaTiO3based2016}) &
  1   (\cite{yanOptimizationThermalConductivity2020}) &
  0 \\
\acrshort{svm} &
  3   (\cite{balachandranDatadrivenDesignB202020,balachandranPredictingDisplacementsOctahedral2017,chenMachineLearningAssisted2020}) &
  12   (\cite{balachandranExperimentalSearchHightemperature2018,caoHowOptimizeMaterials2018,gzylHalfHeuslerStructuresFullHeusler2020,gzylSolvingColoringProblem2019,kauweMachineLearningPrediction2018,oliynykDisentanglingStructuralConfusion2017,raccugliaMachinelearningassistedMaterialsDiscovery2016,tehraniMachineLearningDirected2018,wenMachineLearningAssisted2019,yanOptimizationThermalConductivity2020,zhuoEvaluatingThermalQuenching2020,zhuoIdentifyingEfficientThermally2018}) &
  1   (\cite{yuanAcceleratedDiscoveryLarge2018}) \\
\acrshort{sr} &
  1   (\cite{wengSimpleDescriptorDerived2020}) &
  0 &
  0 \\
\acrshort{rf} &
  1   (\cite{wahabMachinelearningassistedFabricationBayesian2020}) &
  4   (\cite{kauweMachineLearningPrediction2018,oliynykHighThroughputMachineLearningDrivenSynthesis2016,raccugliaMachinelearningassistedMaterialsDiscovery2016,renAcceleratedDiscoveryMetallic2018}) &
  1   (\cite{gaultoisPerspectiveWebbasedMachine2016}) \\
\acrshort{dt} &
  0 &
  2   (\cite{raccugliaMachinelearningassistedMaterialsDiscovery2016,wenMachineLearningAssisted2019}) &
  1   (\cite{meredigCombinatorialScreeningNew2014}) \\
Ensemble &
  0 &
  1   (\cite{gzylHalfHeuslerStructuresFullHeusler2020}) &
  0 \\
\acrshort{ann} &
  0 &
  2   (\cite{wenMachineLearningAssisted2019,yanOptimizationThermalConductivity2020}) &
  1   (\cite{parkDevelopingImprovedCrystal2020}) \\
\acrshort{lasso} &
  0 &
  1   (\cite{buciorEnergybasedDescriptorsRapidly2019}) &
  0 \\
\acrshort{lr} &
  0 &
  3   (\cite{kauweMachineLearningPrediction2018,raccugliaMachinelearningassistedMaterialsDiscovery2016,wenMachineLearningAssisted2019}) &
  0 \\
\acrshort{pr} &
  0 &
  1   (\cite{wenMachineLearningAssisted2019}) &
  0 \\
\acrshort{pls} &
  0 &
  1   (\cite{gzylHalfHeuslerStructuresFullHeusler2020}) &
  0 \\ \hline
\end{tabular}
\end{table}

==> tables/tab-summary.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{longtable}{@{}|l|l|l|l|l|l|l|@{}}
\caption{Tags of all computationally and experimentally validated papers in this review.}
\label{tab:summary}\\
\toprule
Cites &
  C/E? &
  Size &
  ML Type &
  Material &
  Classification &
  Regression \\* \midrule
\endhead
%
\cite{balachandranExperimentalSearchHightemperature2018} &
  E &
  101-10000 &
  \begin{tabular}[c]{@{}l@{}}AD\\ SVM\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Perovskite\\ xBi[MeMeO3]-PbTiO3\end{tabular} &
  Good phase diagram regions &
  high ferro electric curie-Tc \\* \midrule
\cite{beraIntegratedComputationalMaterials2014} &
  E &
  1-100 &
  \begin{tabular}[c]{@{}l@{}}By hand XY plot\\ by hand radar chart\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}SnSe-Ag dopant\\ SnS\end{tabular} &
  High thermoelectric power factor &
   \\* \midrule
\cite{buciorEnergybasedDescriptorsRapidly2019} &
  E &
  \begin{tabular}[c]{@{}l@{}}101-10000 \\ 10000+\end{tabular} &
  Lasso &
  \begin{tabular}[c]{@{}l@{}}hydrogen storage\\ metal organic frameworks\end{tabular} &
   &
  gas uptake \\* \midrule
\cite{caoHowOptimizeMaterials2018} &
  E &
  101-10000 &
  \begin{tabular}[c]{@{}l@{}}DoE\\ SVM\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}organic photovoltaics\\ PDCTBT:PC71\end{tabular} &
   &
  power conversion efficiency \\* \midrule
\cite{chenMachineLearningAssisted2020} &
  E &
  1-100 &
  \begin{tabular}[c]{@{}l@{}}multi objective\\ orthogonal design\\ pare to front vector\\ SVM\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Mg(6wt)Zn(2wt)RE\\ Mg alloy\end{tabular} &
   &
  \begin{tabular}[c]{@{}l@{}}Ductility\\ yield strength\end{tabular} \\* \midrule
\cite{gaultoisPerspectiveWebbasedMachine2016} &
  E &
  10000+ &
  RF &
  \begin{tabular}[c]{@{}l@{}}Gd12Er12Co5Bi\\ thermoelectric\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}high band gap\\ high electrical conductivity\\ high seeback\\ low thermal conductivity\\ promising thermoelectrics\end{tabular} &
   \\* \midrule
\cite{gzylHalfHeuslerStructuresFullHeusler2020} &
  E &
  101-10000 &
  \begin{tabular}[c]{@{}l@{}}ensemble\\ kNN\\ partial LS\\ SVM\\ synthetic minority oversampling\end{tabular} &
   &
  half heusler &
   \\* \midrule
\cite{hommaOptimizationHeterogeneousTernary2020} &
  E &
  1-100 &
  \begin{tabular}[c]{@{}l@{}}AD\\ Bayesian\\ GPR\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Li-ion battery electrolyte\\ Li3PO4-Li3BO3-Li2SO4\end{tabular} &
   &
  Li-ion conductivity \\* \midrule
\cite{houMachineLearningAssistedDevelopmentTheoretical2019} &
  E &
  1-100 &
  \begin{tabular}[c]{@{}l@{}}Bayesian\\ GPR\end{tabular} &
  AlFeSi &
   &
  thermoelectric power factor \\* \midrule
\cite{iwasakiIdentificationAdvancedSpindriven2019} &
  E &
  1-100 &
  \begin{tabular}[c]{@{}l@{}}Bayesian\\ Bayesian FAB/HMEs\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}CoPtN\\ spin thermoelectric\end{tabular} &
   &
  thermopower \\* \midrule
\cite{kauweMachineLearningPrediction2018} &
  E &
  101-10000 &
  \begin{tabular}[c]{@{}l@{}}LinR\\ RF\\ SVM\end{tabular} &
  solid inorganics &
   &
  heat capacity \\* \midrule
\cite{liEfficientOptimizationPerformance2018} &
  E &
  1-100 &
  \begin{tabular}[c]{@{}l@{}}Bayesian\\ GPR\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}CZTSSe\\ solar cell\end{tabular} &
   &
  \begin{tabular}[c]{@{}l@{}}optimal dope ratio\\ solar cell efficiency\end{tabular} \\* \midrule
\cite{mansouritehraniMachineLearningDirected2018} &
  E &
  101-10000 &
  SVM &
  super hard materials &
   &
  highest bulk shear modulous \\* \midrule
\cite{oliynykDisentanglingStructuralConfusion2017} &
  E &
  101-10000 &
  \begin{tabular}[c]{@{}l@{}}CR-FS\\ SVM\\ SVM classification\end{tabular} &
  crystalline inorganic solid &
  crystal structure of ABC phase &
   \\* \midrule
\cite{oliynykHighThroughputMachineLearningDrivenSynthesis2016} &
  E &
  101-10000 &
  RF &
  \begin{tabular}[c]{@{}l@{}}spintronic\\ thermoelectric\end{tabular} &
  Heusler vs. non Heusler &
   \\* \midrule
\cite{raccugliaMachinelearningassistedMaterialsDiscovery2016} &
  E &
  101-10000 &
  \begin{tabular}[c]{@{}l@{}}Decision tree\\ kNN\\ LinR\\ RF\\ SVM\\ SVM\_best\end{tabular} &
  Inorganic organic hybrid &
   &
   \\* \midrule
\cite{renAcceleratedDiscoveryMetallic2018} &
  E &
  101-10000 &
  \begin{tabular}[c]{@{}l@{}}outside of dataset\\ RF\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}CoVZr\\ metallic glass\end{tabular} &
  metallic glasses &
   \\* \midrule
\cite{rickmanMaterialsInformaticsScreening2019} &
  E &
  1-100 &
  \begin{tabular}[c]{@{}l@{}}CCA\\ EA\end{tabular} &
  high entropy alloys &
   &
  hardness \\* \midrule
\cite{wahabMachinelearningassistedFabricationBayesian2020} &
  E &
  1-100 &
  \begin{tabular}[c]{@{}l@{}}AD\\ Bayesian\\ GPR\\ RF\end{tabular} &
  graphene &
   &
  raman GD ratio \\* \midrule
\cite{wakabayashiMachinelearningassistedThinfilmGrowth2019} &
  E &
  1-100 &
  \begin{tabular}[c]{@{}l@{}}AD\\ Bayesian\\ GPR\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}ferromagnetic\\ SrRuO3\end{tabular} &
   &
  residual resistivity ratio \\* \midrule
\cite{wengSimpleDescriptorDerived2020} &
  E &
  1-100 &
  \begin{tabular}[c]{@{}l@{}}pareto\\ SR\end{tabular} &
  oxide perovskites &
   &
  OER \\* \midrule
\cite{xueAcceleratedSearchBaTiO3based2016} &
  E &
  101-10000 &
  \begin{tabular}[c]{@{}l@{}}Bayesian\\ Bayesian Landau-Devron\\ DFT\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}BaTiO3based\\ piezoelectric\end{tabular} &
   &
  morphotropic phase boundary \\* \midrule
\cite{yanOptimizationThermalConductivity2020} &
  E &
  101-10000 &
  \begin{tabular}[c]{@{}l@{}}ANN\\ Bayesian\\ GBDT\\ GPR\\ SVM\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}UO2-Mo\\ nuclear\end{tabular} &
   &
  thermal conductivity \\* \midrule
\cite{yuanAcceleratedDiscoveryLarge2018} &
  E &
  10000+ &
  \begin{tabular}[c]{@{}l@{}}DFT\\ SVM\end{tabular} &
  BaTiO3based &
  strain &
   \\* \midrule
\cite{zhangNotJustPar2018} &
  E &
   &
  \begin{tabular}[c]{@{}l@{}}RF\\ thermo rec engine\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}intermetallics\\ quaternary germanides\end{tabular} &
   &
  \begin{tabular}[c]{@{}l@{}}heat capacity\\ thermal conductivity\end{tabular} \\* \midrule
\cite{zhuoEvaluatingThermalQuenching2020} &
  E &
  101-10000 &
  \begin{tabular}[c]{@{}l@{}}RFE\\ SVM\end{tabular} &
  inorganic phosphors &
   &
  thermal quench temp \\* \midrule
\cite{zhuoIdentifyingEfficientThermally2018} &
  E &
  101-10000 &
  \begin{tabular}[c]{@{}l@{}}DFT\\ SVM\end{tabular} &
  phosphor host crystals &
   &
  debye temp \\* \midrule
\cite{meredigCombinatorialScreeningNew2014} &
  C &
  10000+ &
  \begin{tabular}[c]{@{}l@{}}decision tree\\ heuristic\end{tabular} &
  ternary compounds &
  thermodynamic stability &
  formation energy \\* \midrule
\cite{talapatraAutonomousEfficientExperiment2018} &
  C &
  1-100 &
  \begin{tabular}[c]{@{}l@{}}bayesian\\ GPR\\ ID\end{tabular} &
  MAX ternary cabride nitride &
   &
   \\* \midrule
\cite{balachandranDatadrivenDesignB202020} &
  C &
  1-100 &
  SVM &
  \begin{tabular}[c]{@{}l@{}}B20 alloys\\ spintronics\end{tabular} &
   &
  helical transition temperature \\* \midrule
\cite{balachandranPredictingDisplacementsOctahedral2017} &
  C &
  1-100 &
  SVM &
  \begin{tabular}[c]{@{}l@{}}ferroelectric\\ perovskite\end{tabular} &
   &
  octahedral cation displacement \\* \midrule
\cite{balachandranLearningDataDesign2017} &
  C &
  1-100 &
  \begin{tabular}[c]{@{}l@{}}bootstrap\\ decision tree\\ PCA\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}layered ruddlesden popper oxides \\ noncentro symmetric\end{tabular} &
  noncentro symmetric &
   \\* \midrule
\cite{parkDevelopingImprovedCrystal2020} &
  C &
  10000+ &
  \begin{tabular}[c]{@{}l@{}}ANN\\ GNN\end{tabular} &
  ThCR2Si2 &
   &
  Formation energy \\* \midrule
\cite{sekoMatrixTensorbasedRecommender2018} &
  C &
  101-10000 &
  \begin{tabular}[c]{@{}l@{}}CPD\\ NMF\\ recommender\\ SVD\\ tucker \\ decomposition\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}inorganic crystals\\ ternary compounds\end{tabular} &
  chemically relevant compositions &
   \\* \bottomrule
\end{longtable}
